A Game-Theoretic Analysis of User Behaviors in Crowdsourced Wireless Community Networks

A crowdsourced wireless community network can effectively alleviate the limited coverage issue of Wi-Fi access points (APs), by encouraging individuals (users) to share their private residential Wi-Fi APs with each other. This paper presents the first study on the users' joint membership selection and network access problem in such a network. Specifically, we formulate the problem as a two-stage dynamic game: Stage I corresponds to a membership selection game, in which each user chooses his membership type; Stage II corresponds to a set of network access games, in each of which each user decides his WiFi connection time on the AP at his current location. We analyze the Subgame Perfect Equilibrium (SPE) systematically, and study whether and how best response dynamics can reach the equilibrium. Through numerical studies, we further explore how the equilibrium changes with the users' mobility patterns and network access evaluations. We show that a user with a more popular home location, a smaller travel time, or a smaller network access evaluation is more likely to choose a specific type of membership called Bill. We further demonstrate how the network operator can optimize its pricing and incentive mechanism based on the game equilibrium analysis in this work.

==> Section_app.tex <==

\newpage


\appendices


\section{}

\subsection{Proof of Lemma \ref{lemmaBRLinus}} \label{applemmaBRLinus}

\begin{proof}
If user $i$ is a Linus, his payoff on AP $k$ can be derived from Eq. \eqref{payoffLinus}, which is an increasing function of $\sigma_{i,k}$.
Hence, regardless of other users' strategies, a Linus-type user $i$'s best response is always to choose the maximum network access time, i.e.,
$\sigma_{i,k}^\ast = 1$.
\end{proof}



\subsection{Proof of Lemma \ref{lemmaBRBill}} \label{applemmaBRBill}

\begin{proof}
If user $i$  is a Bill or an Alien, his payoff at AP $k$ can be derived from Eq. \eqref{payoffBill}. Hence, the payoff maximization problem for user $i$ on AP $k$ can be written as follows
\begin{align}
& \displaystyle \max ~~ \rho_i \log(1+\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k}) \cdot \sigma_{i,k}) - p \sigma_{i,k} \notag\\
& \mbox{~s.t.} ~~~~ 0 \leq \sigma_{i,k} \leq 1 \notag\\
& \mbox{~var:} ~~~ \sigma_{i,k} \notag
\end{align}
which is a concave maximization problem. By using the first-order condition, we can derive a Bill-type of Alien user $i$'s best response:
\begin{equation*}
\sigma_{i,k}^\ast = \min\left\{ 1,\max\left\{ \frac{\rho_i}{p}-\frac{1}{\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k})},0 \right\} \right\},
\end{equation*}
which is a function of other users' strategies $\boldsymbol{\sigma}_{-i,k} $.
\end{proof}






\subsection{Proof of Theorem \ref{ExiNEI}} \label{applemmaExiNEI}

\begin{proof}
To prove Theorem \ref{ExiNEI}, we first introduce the Brouwer fixed-point theorem \cite{Brouwer}, 
which states that every continuous mapping $f$ from a compact convex set to itself has a fixed point $z_0$ satisfying $z_0=f(z_0).$

The Nash equilibrium $\boldsymbol{\sigma}_k^\ast=\{\sigma_{i,k}^\ast,\forall i \in \K(k)\}$ is computed by Lemma \ref{lemmaBRLinus} and Lemma \ref{lemmaBRBill}.
Specifically,
\begin{equation*}
\sigma_{i,k}^\ast =\\
\begin{cases}
1, \mbox{ Linus} ~i;
\\
\min\left\{ 1,\max\left\{ \frac{\rho_i}{p}-\frac{1}{\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k})},0 \right\} \right\}, \mbox{ Bill or Alien} ~i.
\end{cases}
\end{equation*}
%each Linus-type user $i$'s best response is $\sigma_{i,k}^\ast=1$,
%and each Bill-type or Alien user $i$'s best response is calculated by the following mapping function:
%$$ \sigma_{i,k}^\ast=\min\left\{ 1,\max\left\{ \frac{\rho_i}{p}-\frac{1}{\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k})},0 \right\} \right\}. $$
This is a continuous mapping from a compact convex set $[0,1]$ to itself, which satisfies the requirement of the Brouwer fixed-point theorem.
Hence, there exists a fixed point $\boldsymbol{\sigma}_k^\ast$ satisfying
\begin{equation*}
\sigma_{i,k}^\ast =\\
\begin{cases}
1, \mbox{ Linus} ~i;
\\
\min\left\{ 1,\max\left\{ \frac{\rho_i}{p}-\frac{1}{\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k}^\ast)},0 \right\} \right\}, \mbox{ Bill or Alien} ~i.
\end{cases}
\end{equation*}
The fixed point $\boldsymbol{\sigma}_k^\ast$ is the Nash equilibrium.
\end{proof}




\subsection{Best Response Update Algorithm for the Network Access Game}\label{appAlg1}

We further design a Best Response Update Algorithm to derive the Nash equilibrium.
The basic idea is as follows.
Given the strategy profile $\boldsymbol{\sigma}_k^t$ at the $t$-th round,
each player compute the corresponding best response.
We denote the best responses of all players by $T(\boldsymbol{\sigma}_k^t)$.
Each user updates the strategy at the $(t+1)$-th round as the best response in $T(\boldsymbol{\sigma}_k^t)$.


\begin{algorithm}[h]
\SetAlgoLined
\KwIn{$\boldsymbol{\sigma}_k^0,\varepsilon . $}
\KwOut{$ \boldsymbol{\sigma}_k^\ast . $}
Set $t = 0$ and $Flag = 0$.\\
\While {$Flag = 0$}{
Calculate $\boldsymbol{\sigma}_k^{t+1}= T(\boldsymbol{\sigma}_k^t)  $.\\
\If{$|\boldsymbol{\sigma}_k^{t+1}-\boldsymbol{\sigma}_k^t|\leq \varepsilon$}{
set $Flag = 1$.
}
Set $t = t+1$.
}
Set $ \boldsymbol{\sigma}_k^\ast=\boldsymbol{\sigma}_k^t. $
\caption{Best Response Update Algorithm}
\label{algo:br1}
\end{algorithm}


\begin{proposition}\label{ConA1}
In the Network Access Game with two players, the sequence generate by the Best Response Update Algorithm linearly converges to the unique Nash equilibrium under the following condition:
$$ c \equiv \frac{R(1)-R(2)}{R(2)^2} < 1 .$$
\end{proposition}

Note that the condition in Proposition \ref{ConA1} is always satisfied for practical WiFi systems \cite{20Q}.




\subsection{Proof of Proposition \ref{UniNEI} and Proposition \ref{ConA1}}\label{appUniNEI}


Assume there are $2$ APs and $1$ Alien in the network, and we study the two-player network access game on AP $2$. The two players are subscriber $1$ and the Alien, and their strategies are $\sigma_{1,2}\in[0,1]$ and $\sigma_{a,2}\in[0,1]$. We have already shown that there exists a Nash equilibrium $(\sigma_{1,2}^\ast,\sigma_{a,2}^\ast)$ where:
\begin{equation*}
\sigma_{1,2}^\ast =\\
\begin{cases}
1, \mbox{ if } ~x_1=0;
\\
\min\left\{ 1,\max\left\{ \frac{\rho_1}{p}-\frac{1}{\bar{r}_{1,2}(\boldsymbol{\sigma}_{a,2}^\ast)},0 \right\} \right\}, \mbox{ if } ~x_1=1;
\end{cases}
\end{equation*}
and
$$\sigma_{a,2}^\ast = \min\{1,\max\{\frac{\rho_a}{p}-\frac{1}{\bar{r}_{a,2}(\sigma_{1,2}^\ast)},0\}\}.$$
Here the expected data rates of subscriber $1$ and the Alien are
\begin{align}
& \bar{r}_{1,2}(\sigma_{a,2}^\ast)=(1-\sigma_{a,2}^\ast)R(1)+\sigma_{a,2}^\ast R(2), \notag \\
& \bar{r}_{a,2}(\sigma_{1,2}^\ast)=(1-\sigma_{1,2}^\ast)R(1)+\sigma_{1,2}^\ast R(2). \notag
\end{align}

Proposition \ref{UniNEI} and Proposition \ref{ConA1} claim that (i) the Nash equilibrium $(\sigma_{1,2}^\ast,\sigma_{a,2}^\ast)$ is unique and (ii) the sequence $\{(\sigma_{1,2}^t,\sigma_{a,2}^t)\}$ generated by Algorithm \ref{algo:br1} linearly converges to the unique Nash equilibrium $(\sigma_{1,2}^\ast,\sigma_{a,2}^\ast)$
as long as
$$ c \equiv \frac{R(1)-R(2)}{R(2)^2} < 1 .$$

Note that the condition required above is alwasy satisfied for practical WiFi \cite{20Q}.

\begin{proof}
If subscriber $1$ chooses to be a Linus, i.e., $x_1=0$, then $\sigma_{1,2}^\ast=1$, and
$$\sigma_{a,2}^\ast = \min\{1,\max\{\frac{\rho_a}{p}-\frac{1}{\bar{r}_{a,2}(R(2)},0\}\}.$$
The Nash equilibrium is unique and we can directly derive it.

If subscriber $1$ chooses to be a Bill, i.e., $x_1=1$, then we have the following discussions.

We denote the strategy profile at the $t$-th round as $\boldsymbol{\sigma}_2^t$, and each user updates the strategy at the $(t+1)$-th round. 
We denote the strategy profile at the $(t+1)$-th round as $\boldsymbol{\sigma}_2^{t+1}$.
We consider the following cases:

\textbf{A}: If $\frac{\rho_1}{p}-\frac{1}{R(1)}<0$, then $\sigma_{1,2}^t=0$ and
$$ \sigma_{a,2}^t=\frac{\rho_a}{p}-\frac{1}{R(1)} $$
for all $t$.

\textbf{B}: If $\frac{\rho_1}{p}-\frac{1}{R(2)}>1$, then $\sigma_{1,2}^t=1$ and
$$ \sigma_{a,2}^t=\frac{\rho_a}{p}-\frac{1}{R(2)} $$
for all $t$.

\textbf{C}: If $\frac{\rho_1}{p}-\frac{1}{R(1)}\geq 0$ and $\frac{\rho_1}{p}-\frac{1}{R(2)}\leq 1$, then we further consider the following three subcases:
\begin{itemize}
\item If $\frac{\rho_a}{p}-\frac{1}{R(1)}<0$, then $\sigma_{a,2}^t=0$ and
$$ \sigma_{1,2}^t=\frac{\rho_1}{p}-\frac{1}{R(1)} $$
for all $t$.
\item If $\frac{\rho_a}{p}-\frac{1}{R(2)}>1$, then $\sigma_{a,2}^t=1$ and
$$ \sigma_{1,2}^t=\frac{\rho_1}{p}-\frac{1}{R(2)} $$
for all $t$.
\item If $\frac{\rho_a}{p}-\frac{1}{R(1)}\geq 0$ and $\frac{\rho_a}{p}-\frac{1}{R(2)}\leq 1$, then we have
\begin{align}
& \sigma_{1,2}^{t+1} = \frac{\rho_1}{p}-\frac{1}{\bar{r}_{1,2}(\sigma_{a,2}^t)}, \notag \\
& \sigma_{a,2}^{t+1} = \frac{\rho_a}{p}-\frac{1}{\bar{r}_{a,2}(\sigma_{1,2}^t)}. \notag
\end{align}
\end{itemize}

Therefore, we have:
\begin{align}
& |\sigma_{1,2}^{t+1}-\sigma_{1,2}^\ast| \notag \\
=& | \frac{1}{\bar{r}_{1,2}(\sigma_{a,2}^t)} - \frac{1}{\bar{r}_{1,2}(\sigma_{a,2}^\ast)} | \notag \\
=& | \frac{1}{R(1)-\sigma_{a,2}^\ast (R(1)-R(2))} - \frac{1}{R(1)-\sigma_{a,2}^t (R(1)-R(2))} | \notag \\
=& \frac{[R(1)-R(2)]\cdot |\sigma_{a,2}^t-\sigma_{a,2}^\ast|}{[R(1)-\sigma_{a,2}^\ast(R(1)-R(2))][R(1)-\sigma_{a,2}^t(R(1)-R(2))]}  \notag \\
\leq & c \cdot |\sigma_{a,2}^t-\sigma_{a,2}^\ast|, \notag
\end{align}
and similarly
$$ |\sigma_{a,2}^{t+1}-\sigma_{a,2}^\ast| \leq c |\sigma_{1,2}^t-\sigma_{1,2}^\ast|.$$

The above shows that
$$\| \boldsymbol{\sigma}_2^{t+1}-\boldsymbol{\sigma}_2^\ast \| \leq c \| \boldsymbol{\sigma}_2^t-\boldsymbol{\sigma}_2^\ast \|$$
for all $t>0$, which further implies that $\{(\sigma_{1,2}^t,\sigma_{a,2}^t)\}$ converges to the unique Nash equilibrium $(\sigma_{1,2}^\ast,\sigma_{a,2}^\ast)$ and the convergence rate is linear.
\end{proof}









\subsection{Proof of Lemma \ref{lemmaMS}}\label{applemmaMS}

\begin{proof}
We first prove the necessity.
If $f_i(\boldsymbol{x}_{-i}^\ast) < 0$, the best membership for subscriber $i$ is $x_i^\ast = 0$ (Linus), hence $(2x_i^\ast-1)\cdot f_i(\boldsymbol{x}_{-i}^\ast) = - f_i(\boldsymbol{x}_{-i}^\ast)> 0 $.
If $f_i(\boldsymbol{x}_{-i}^\ast) > 0$, the best membership for subscriber $i$ is $x_i^\ast = 1$ (Bill), hence $(2x_i^\ast-1)\cdot f_i(\boldsymbol{x}_{-i}^\ast) =  f_i(\boldsymbol{x}_{-i}^\ast)> 0 $.
Then we prove the sufficiency.
Suppose $f_i(\boldsymbol{x}_{-i}^\ast) < 0$. Then the desired $x_i^*$ that satisfies the condition in Lemma \ref{lemmaMS} is $x_i^* = 0$, which is obviously the best strategy of subscriber $i$.
Suppose $f_i(\boldsymbol{x}_{-i}^\ast) > 0$. Then the desired $x_i^*$ that satisfies the condition in Lemma \ref{lemmaMS} is $x_i^* = 1$, which is also the best strategy of subscriber $i$.
\end{proof}




\subsection{Proof of Proposition \ref{lemmaETA}}\label{app2}

\rev{To be added.}

%The condition
%$$ \eta_{i,i}> 1- \frac{A_i}{\rho_i \log (1+R(1))+p} $$
%is equal to
%$$ A_i > \sum_{k \neq i} \eta_{i,k} (\rho_i \log(1+R(1))+p). $$
%Hence, the payoff difference under the membership Bill and Linus is:
%\begin{align}
%& V_i(1,\boldsymbol{x}_{-i})-V_i(0,\boldsymbol{x}_{-i}) \notag \\
%= & A_i+\delta p \sum_{k\neq i} x_k \eta_{k,i} \sigma_{k,i} + \sum_{k\neq i} \eta_{i,k}(\rho_i \log(1+\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k})\sigma_{i,k})\notag \\
%& -p\sigma_{i,k}) - \sum_{k\neq i} \eta_{i,k}\rho_i \log(1+\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k})) \notag \\
%\geq & A_i - \sum_{k\neq i} \eta_{i,k}\left(\rho_i \log(\frac{1+\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k})}{1+\bar{r}_{i,k}(\boldsymbol{\sigma}_{-i,k})\sigma_{i,k}})+p \sigma_{i,k} \right) \notag \\
%\geq & A_i - \sum_{k \neq i} \eta_{i,k} (\rho_i \log(1+R(1))+p) > 0. \notag
%\end{align}
%AP owner $i$'s payoff of being a Bill is always larger than that of being a Linus. Hence, choosing Bill is a strictly dominant strategy.





\subsection{Mixed-Strategy Update Algorithm for the Membership Selection Game}\label{appAlg2}

We further design a Mixed-Strategy Update Algorithm to calculate the mixed-strategy Nash equilibrium.
The basic idea is as follows.
First, given the mixed strategy profile $\boldsymbol{\alpha}^t$ at the $t$-th round, each player compute the corresponding expected payoff when choosing to be Bill (i.e., $\widetilde{V}_i(1,\boldsymbol{\alpha}_{-i})$) or to be Linus (i.e., $\widetilde{V}_i(0,\boldsymbol{\alpha}_{-i})$).
Then, each player updates his mixed strategy at the $(t+1)$-th round according to the following \emph{smoothed}
best response method \cite{Game-Learning}:
$$
\alpha_i^{t+1}=\frac{ e^{  \widetilde{V}_i(1,\boldsymbol{\alpha}_{-i}) /\gamma }}{ e^{  \widetilde{V}_i(1,\boldsymbol{\alpha}_{-i}) /\gamma }+e^{  \widetilde{V}_i(0,\boldsymbol{\alpha}_{-i}) /\gamma}} ,
$$
where $\gamma $ is a parameter that determines the degree to which the function deviates from the true best response (a larger $\gamma$ implies that the player is more likely to act randomly).


\begin{algorithm}[h]
\SetAlgoLined
\KwIn{$\boldsymbol{\alpha}^0,\gamma . $}
\KwOut{$ \boldsymbol{\alpha}^\ast . $}
Set $t = 0$ and $Flag = 0$.\\
\While {$Flag = 0$}{
\For{$i=1:K$}{
Calculate $\widetilde{V}_i(1,\boldsymbol{\alpha}_{-i})$ and $\widetilde{V}_i(0,\boldsymbol{\alpha}_{-i})$;
\\
Update $\alpha_i^{t+1}=\frac{ e^{  \widetilde{V}_i(1,\boldsymbol{\alpha}_{-i}) /\gamma }}{ e^{  \widetilde{V}_i(1,\boldsymbol{\alpha}_{-i}) /\gamma }+e^{  \widetilde{V}_i(0,\boldsymbol{\alpha}_{-i}) /\gamma}} $.
}
\If{$|\boldsymbol{\alpha}^{t+1}-\boldsymbol{\alpha}^t|\leq 10^{-6}$}{
set $Flag = 1$.
}
Set $t = t+1$.
}
Set $ \boldsymbol{\alpha}^\ast=\boldsymbol{\alpha}^t. $
\caption{Mixed Strategy Update Algorithm}
\label{algo:br}
\end{algorithm}

(\com{Proof of convergence, under limited scenarios? })


\subsection{Location-Dependent Pricing Scheme}


\rev{
We then numerically study whether and how much the location-dependent pricing scheme can increase the operator's revenue. In this simulation, we fixed the revenue sharing ratio at $\delta=0.63$ (i.e., the ratio under the optimal location-independent pricing and incentive scheme).
Figure \ref{fig:RevenuePrice} presents the operator's revenue under three different pricing schemes.
\emph{Yellow Bar}: The operator sets a single price $p=0.58$ (i.e., the price under the optimal location-independent pricing and incentive scheme), and can get an average revenue of $11.40$ as illustrated in Figure \ref{fig:Revenue}.
\emph{Light Green Bar}: The operator sets a location-dependent pricing scheme with three prices $\boldsymbol{p}=[0.3,0.6,1.2]$ (assigned to different locations properly), and can get an average revenue of $19.40$.
\emph{Dark Green Bar}: The operator sets a location-dependent pricing scheme with six prices $\boldsymbol{p}=[0.3,0.5,0.6,0.8,1.0,1.2]$ (assigned to different locations properly), and can get an average revenue of $22.90$.
Hence, with the (even not optimal) location-dependent pricing schemes, the operator can increase its revenue up to $70\%$ and $100\%$.
This shows the potential of location-dependent pricing scheme in increasing the  operator's revenue.}

\begin{figure}
  %\vspace{-5mm}
  \centering
   \includegraphics[width=0.35\textwidth]{fig/RevenuePrice3}
   %\vspace{-3mm}
  \caption{Operator's Revenue under Location-Dependent Pricing}\label{fig:RevenuePrice}
  %\vspace{-5mm}
\end{figure}



==> Section_simu.tex <==


\section{Simulation Results}\label{sec:simu}


%(\com{Besides simulating our game equilibrium, it would be useful to simulate other benchmarks, for several reasons:
%- Some readers always want to see comparison.
%- The game equilibrium is assuming complete information, which is difficult to get in practice. Based on our game analysis, especially Prop 2, Prop 3, and Figure 5, it is possible to design some heuristic algorithm that relies only on local information without global information? This can serve as a good benchmark.
%- What about centralized benchmark? If the network operator can choose the memberships for all users to maximize users' total payoffs, how will our results compare with that benchmark? This will be a numerical study of the Price of Anarchy. })

In this section, we numerically study how the network access valuation parameter $\rho_i$ and the mobility probability vector $\boldsymbol{\eta}_i$ influence subscriber $i$'s membership selection decision, given other system parameters fixed.

In Section \ref{subsec:small}, we will first simulate a small network with $2$ APs and $1$ Alien, to gain insights of a single user's best choice.
Then, in Section \ref{subsec:large}, we simulate a large network with $100$ APs to understand the system-level performance.


\subsection{A Small Network Example}\label{subsec:small}

We simulate a small network with $2$ subscribers (each owns an AP) and $1$ Alien.
We study how subscriber $1$'s network access valuation parameter $\rho_1$ and his probability of staying at home $\eta_{1,1}$ affects his membership selection.

We assume the revenue share ratio $\delta=0.5$. The price at both APs is $p=1$.
The mobility probability vectors of subscriber $2$ and the Alien are same: $\boldsymbol{\eta}_2=\boldsymbol{\eta}_a=[1/3,1/3,1/3]$.
We assume that $\rho_1 \in [0,1]$. Subscriber $1$ stays at home with probability $\eta_{1,1}$, and travels to AP $2$ and outside the Wi-Fi coverage with a same probability $\eta_{1,2}=\eta_{1,0}=(1-\eta_{1,1})/2$.

Figure \ref{fig:Parameter} shows subscriber $1$'s membership selection decision in the equilibrium in Definition \ref{NEImixed} in Section \ref{subsec:mexed}, under different $\rho_i \in [0,1]$ and $\eta_{1,1} \in [0,1]$.
The color represents the value of $\alpha_1$, which is subscriber $1$'s probability of choosing to be a Bill.
The dark blue color corresponds to $\alpha_1=1$, and light green color corresponds to $\alpha_1=0$.
The colors in between represent a mixed strategy of $\alpha_1\in (0,1)$.
As shown in the colorbar, the color which changes from light blue to dark blue represents the exact value of $\alpha_1$ changing from $0$ to $1$.

As we can see in Figure \ref{fig:Parameter}, when $\eta_{1,1}$ is large enough (i.e., larger than $0.82$), i.e., subscriber $1$ stays at home most of the time, his will always choose to be a Bill with the probability $\alpha_1=1$, independent of subscriber $2$'s membership decision.
As $\eta_{1,1}$ becomes smaller and $\rho_1$ becomes larger, the performance and payment during roaming becomes increasingly important, so subscriber $1$ starts to choose a mixed strategy with a smaller number of $\alpha_1$.
When $\eta_{1,1}$ is small enough and $\rho_1$ is large enough, e.g., the right bottom corner of Figure \ref{fig:Parameter}, he will always choose to be a Linus with a probability $1-\alpha_1=1$.

\begin{figure}
  %\vspace{-5mm}
  \centering
   \includegraphics[width=0.4\textwidth]{fig/SmallNetwork}
   %\vspace{-3mm}
  \caption{Membership Decision under Different Parameters}\label{fig:Parameter}
  %\vspace{-5mm}
\end{figure}

\com{The color for $\alpha_1=1$ is clear, but the color for $\alpha_1=0$ is not clear from this figure.
Can we adjust the color, so that the colors for both extremes are clearly different from the middle colors? }


\subsection{Simulation Results for Large Network}\label{subsec:large}

In this subsection, we simulation a larger network with $100$ APs.


\subsubsection{Impact of Location Popularity}

We first study how the location popularity of an AP affects the subscriber's membership selection decision. The location popularity is measured by the probabilities of users showing up at that location. For simplicity, we assume that all the users show up at each location with the same probability, and the location popularity of the APs that are indexed from $1$ to $100$ uniformly increases.

Figure \ref{fig:LP} shows each subscriber's membership selection decision. The three curves represent three different values of the subscriber's network access valuation parameter $\rho_i$. Under a given $\rho_i$, the subscriber's probability of choosing to be a Bill increases with his AP location popularity. The reason is that a subscriber whose AP is located at a more popular location can earn more revenue from other Bills and Aliens. For a particular subscriber (a fixed AP index), as his network access valuation $\rho_i$ increases, his probability of choosing to be a Bill decreases. This is because he cares more about the network access benefit when roaming and is more willing to be a Linus to enjoy free access and consume more data during roaming.


\begin{figure}
  %\vspace{-5mm}
  \centering
   \includegraphics[width=0.4\textwidth]{fig/Location2}
   %\vspace{-3mm}
  \caption{Membership Decisions of All Subscribers}\label{fig:LP}
  %\vspace{-5mm}
\end{figure}




\subsubsection{Operator's Revenue}

Finally we discuss how the operator can utilize the analysis in this paper to optimize its revenue.
In particular, the operator can optimize $p$ and $\delta$, based on the users' equilibrium membership selection and network access decisions.

Figure \ref{fig:Revenue} presents contours of the operator's revenue with respect to $p$ and $\delta$.
In this case, the optimal price and revenue sharing ratio for the operator are $p^* = 0.62$ and $\delta^* = 56\%$, which lead to an average revenue of $11.4$ (per time slot) for the operator.
We can further see that the operator's maximum revenue is close to zero under the extreme case without incentive (i.e., $\delta = 0 \%$), and is around $8$ \com{not clear from the figure. Can we change the figure so that both 0 and 8 are part of the contours? } under another extreme case with the maximum incentive (i.e., $\delta =100\%$).
\com{what are the optimal prices under both extreme cases? }
\com{explain the intuition why these extreme cases (especially the case without incentive) is so bad. }


\begin{figure}
  %\vspace{-5mm}
  \centering
   \includegraphics[width=0.35\textwidth]{fig/Revenue2}
   %\vspace{-3mm}
  \caption{Operator's Revenue}\label{fig:Revenue}
  %\vspace{-5mm}
\end{figure}


